Measurement of $P_T$-weighted Sivers asymmetries in leptoproduction of hadrons

The transverse spin asymmetries measured in semi-inclusive leptoproduction of hadrons, when weighted with the hadron transverse momentum $P_T$, allow for the extraction of important transverse-momentum-dependent distribution functions. In particular, the weighted Sivers asymmetries provide direct information on the Sivers function, which is a leading-twist distribution that arises from a correlation between the transverse momentum of an unpolarised quark in a transversely polarised nucleon and the spin of the nucleon. Using the high-statistics data collected by the COMPASS Collaboration in 2010 with a transversely polarised proton target, we have evaluated two types of $P_T$-weighted Sivers asymmetries, which are both proportional to the product of the firsttransverse moment of the Sivers function and of the fragmentation function. The results are compared to the standard unweighted Sivers asymmetries and used to extract the first transverse moments of the Sivers distributions for $u$ and $d$ quarks.

==> Authors2018-Barone-Sbrizzai-Schiavon-Sozzi.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% 2018_auththorlist.tex
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{The COMPASS Collaboration}
\label{app:collab}
\renewcommand\labelenumi{\textsuperscript{\theenumi}~}
\renewcommand\theenumi{\arabic{enumi}}
\begin{flushleft}
M.G.~Alexeev\Irefn{turin_u},
G.D.~Alexeev\Irefn{dubna}, %1
A.~Amoroso\Irefnn{turin_u}{turin_i},
V.~Andrieux\Irefnn{illinois}{saclay},
N.V.~Anfimov\Irefn{dubna}, %2
V.~Anosov\Irefn{dubna}, %3
A.~Antoshkin\Irefn{dubna}, % phd
K.~Augsten\Irefnn{dubna}{praguectu}, %prague
W.~Augustyniak\Irefn{warsaw},
C.D.R.~Azevedo\Irefn{aveiro},
B.~Bade{\l}ek\Irefn{warsawu},
F.~Balestra\Irefnn{turin_u}{turin_i},
M.~Ball\Irefn{bonniskp},
J.~Barth\Irefn{bonnpi},
V.~Barone\Irefnn{alessandria}{turin_i}, % Vincenzo
R.~Beck\Irefn{bonniskp},
Y.~Bedfer\Irefn{saclay},
J.~Bernhard\Irefnn{mainz}{cern},
K.~Bicker\Irefnn{munichtu}{cern},
E.~R.~Bielert\Irefn{cern},
M.~Bodlak\Irefn{praguecu},
P.~Bordalo\Irefn{lisbon}\Aref{a},
F.~Bradamante\Irefnn{triest_u}{triest_i},
A.~Bressan\Irefnn{triest_u}{triest_i},
M.~B\"uchele\Irefn{freiburg},
V.E.~Burtsev\Irefn{tomsk},
W.-C.~Chang\Irefn{taipei},
C.~Chatterjee\Irefn{calcutta},
M.~Chiosso\Irefnn{turin_u}{turin_i},
A.G.~Chumakov\Irefn{tomsk},
S.-U.~Chung\Irefn{munichtu}\Aref{b},
A.~Cicuttin\Irefn{triest_i}\Aref{ictp},
M.L.~Crespo\Irefn{triest_i}\Aref{ictp},
S.~Dalla Torre\Irefn{triest_i},
S.S.~Dasgupta\Irefn{calcutta},
S.~Dasgupta\Irefnn{triest_u}{triest_i},
O.Yu.~Denisov\Irefn{turin_i}\CorAuth,
L.~Dhara\Irefn{calcutta},
S.V.~Donskov\Irefn{protvino},
N.~Doshita\Irefn{yamagata},
Ch.~Dreisbach\Irefn{munichtu},
W.~D\"unnweber\Arefs{r},
R.R.~Dusaev\Irefn{tomsk},
M.~Dziewiecki\Irefn{warsawtu},
A.~Efremov\Irefn{dubna}\Aref{o}, %4
C.~Elia\Irefnn{triest_u}{triest_i},
P.D.~Eversheim\Irefn{bonniskp},
M.~Faessler\Arefs{r},
A.~Ferrero\Irefn{saclay},
M.~Finger\Irefn{praguecu},
M.~Finger~jr.\Irefn{praguecu},
H.~Fischer\Irefn{freiburg},
C.~Franco\Irefn{lisbon},
N.~du~Fresne~von~Hohenesche\Irefnn{mainz}{cern},
J.M.~Friedrich\Irefn{munichtu}\CorAuth,
V.~Frolov\Irefnn{dubna}{cern},   %5
F.~Gautheron\Irefnn{bochum}{illinois},
O.P.~Gavrichtchouk\Irefn{dubna}, %6
S.~Gerassimov\Irefnn{moscowlpi}{munichtu},
J.~Giarra\Irefn{mainz},
I.~Gnesi\Irefnn{turin_u}{turin_i},
M.~Gorzellik\Irefn{freiburg}\Aref{c},
A.~Grasso\Irefnn{turin_u}{turin_i},
A.~Gridin\Irefn{dubna},
M.~Grosse Perdekamp\Irefn{illinois},
B.~Grube\Irefn{munichtu},
%T.~Grussenmeyer\Irefn{freiburg},
A.~Guskov\Irefn{dubna}, %7
D.~Hahne\Irefn{bonnpi},
G.~Hamar\Irefn{triest_i},
D.~von~Harrach\Irefn{mainz},
R.~Heitz\Irefn{illinois},
F.~Herrmann\Irefn{freiburg},
N.~Horikawa\Irefn{nagoya}\Aref{d},
N.~d'Hose\Irefn{saclay},
C.-Y.~Hsieh\Irefn{taipei}\Aref{x},
S.~Huber\Irefn{munichtu},
S.~Ishimoto\Irefn{yamagata}\Aref{e},
A.~Ivanov\Irefnn{turin_u}{turin_i},
%Yu.~Ivanshin\Irefn{dubna},
T.~Iwata\Irefn{yamagata},
M.~Jandek\Irefn{praguectu},
V.~Jary\Irefn{praguectu},
R.~Joosten\Irefn{bonniskp},
P.~J\"org\Irefn{freiburg}\Aref{joerg_adr},
K.~Juraskova\Irefn{praguectu};
E.~Kabu\ss\Irefn{mainz},
F.~Kaspar\Irefn{munichtu},
A.~Kerbizi\Irefnn{triest_u}{triest_i},
B.~Ketzer\Irefn{bonniskp},%\Aref{f},
G.V.~Khaustov\Irefn{protvino},
Yu.A.~Khokhlov\Irefn{protvino}\Aref{g}, %\Aref{v},
Yu.~Kisselev\Irefn{dubna}, %9
F.~Klein\Irefn{bonnpi},
J.H.~Koivuniemi\Irefnn{bochum}{illinois},
V.N.~Kolosov\Irefn{protvino},
K.~Kondo\Irefn{yamagata},
I.~Konorov\Irefnn{moscowlpi}{munichtu},
V.F.~Konstantinov\Irefn{protvino},
A.M.~Kotzinian\Irefn{turin_i}\Aref{yerevan},
O.M.~Kouznetsov\Irefn{dubna}, %10
Z.~Kral\Irefn{praguectu},
M.~Kr\"amer\Irefn{munichtu},
F.~Krinner\Irefn{munichtu},
Z.V.~Kroumchtein\Irefn{dubna}\Deceased, %11
Y.~Kulinich\Irefn{illinois},
F.~Kunne\Irefn{saclay},
K.~Kurek\Irefn{warsaw},
R.P.~Kurjata\Irefn{warsawtu},
%I.I.~Kuznetsov\Irefn{tomsk},
A.~Kveton\Irefn{praguectu},
A.A.~Lednev\Irefn{protvino}\Deceased,
%E.A.~Levchenko\Irefn{tomsk},
S.~Levorato\Irefn{triest_i},
Y.-S.~Lian\Irefn{taipei}\Aref{y},
J.~Lichtenstadt\Irefn{telaviv},
R.~Longo\Irefnn{turin_u}{turin_i},
V.E.~Lyubovitskij\Irefn{tomsk}\Aref{regen},
A.~Maggiora\Irefn{turin_i},
A.~Magnon\Irefn{illinois},
N.~Makins\Irefn{illinois},
N.~Makke\Irefn{triest_i}\Aref{ictp},
G.K.~Mallot\Irefn{cern},
S.A.~Mamon\Irefn{tomsk},
B.~Marianski\Irefn{warsaw},
A.~Martin\Irefnn{triest_u}{triest_i},
J.~Marzec\Irefn{warsawtu},
J.~Matou{\v s}ek\Irefnnn{triest_u}{triest_i}{praguecu},
%H.~Matsuda\Irefn{yamagata},
T.~Matsuda\Irefn{miyazaki},
G.V.~Meshcheryakov\Irefn{dubna}, %12
M.~Meyer\Irefnn{illinois}{saclay},
W.~Meyer\Irefn{bochum},
Yu.V.~Mikhailov\Irefn{protvino},
M.~Mikhasenko\Irefn{bonniskp},
E.~Mitrofanov\Irefn{dubna},  % phd
N.~Mitrofanov\Irefn{dubna},  % phd
Y.~Miyachi\Irefn{yamagata},
A.~Moretti\Irefn{triest_u},
A.~Nagaytsev\Irefn{dubna}, %13
D.~Neyret\Irefn{saclay},
J.~Nov{\'y}\Irefnn{praguectu}{cern},
W.-D.~Nowak\Irefn{mainz},
G.~Nukazuka\Irefn{yamagata},
A.S.~Nunes\Irefn{lisbon},
A.G.~Olshevsky\Irefn{dubna}, %14
I.~Orlov\Irefn{dubna}, % phd
M.~Ostrick\Irefn{mainz},
D.~Panzieri\Irefn{turin_i}\Aref{turin_p},
B.~Parsamyan\Irefnn{turin_u}{turin_i},
S.~Paul\Irefn{munichtu},
J.-C.~Peng\Irefn{illinois},
F.~Pereira\Irefn{aveiro},
M.~Pe{\v s}ek\Irefn{praguecu},
M.~Pe{\v s}kov\'a\Irefn{praguecu},
D.V.~Peshekhonov\Irefn{dubna}, %15
N.~Pierre\Irefnn{mainz}{saclay},
S.~Platchkov\Irefn{saclay},
J.~Pochodzalla\Irefn{mainz},
V.A.~Polyakov\Irefn{protvino},
J.~Pretz\Irefn{bonnpi}\Aref{h},
M.~Quaresma\Irefn{lisbon},
C.~Quintans\Irefn{lisbon},
S.~Ramos\Irefn{lisbon}\Aref{a},
C.~Regali\Irefn{freiburg},
G.~Reicherz\Irefn{bochum},
C.~Riedl\Irefn{illinois},
D.I.~Ryabchikov\Irefnn{protvino}{munichtu}, %\Aref{v},
A.~Rybnikov\Irefn{dubna}, % phd
A.~Rychter\Irefn{warsawtu},
R.~Salac\Irefn{praguectu},
V.D.~Samoylenko\Irefn{protvino},
A.~Sandacz\Irefn{warsaw},
S.~Sarkar\Irefn{calcutta},
I.A.~Savin\Irefn{dubna}\Aref{o}, %16
T.~Sawada\Irefn{taipei},
G.~Sbrizzai\Irefnn{triest_u}{triest_i}\CorAuth,
P.~Schiavon\Irefnn{triest_u}{triest_i}, %for wa paper only
H.~Schmieden\Irefn{bonnpi},
E.~Seder\Irefn{saclay},
A.~Selyunin\Irefn{dubna}, % phd
L.~Silva\Irefn{lisbon},
L.~Sinha\Irefn{calcutta},
S.~Sirtl\Irefn{freiburg},
M.~Slunecka\Irefn{dubna}, %17
J.~Smolik\Irefn{dubna}, %18
F.~Sozzi\Irefn{triest_i}, %for wa paper only
A.~Srnka\Irefn{brno},
D.~Steffen\Irefnn{cern}{munichtu},
M.~Stolarski\Irefn{lisbon},
O.~Subrt\Irefnn{cern}{praguectu},
M.~Sulc\Irefn{liberec},
H.~Suzuki\Irefn{yamagata}\Aref{d},
A.~Szabelski\Irefnnn{triest_u}{triest_i}{warsaw} %also {triest_i}
T.~Szameitat\Irefn{freiburg}\Aref{c},
P.~Sznajder\Irefn{warsaw},
M.~Tasevsky\Irefn{dubna}, %19
S.~Tessaro\Irefn{triest_i},
F.~Tessarotto\Irefn{triest_i},
A.~Thiel\Irefn{bonniskp},
J.~Tomsa\Irefn{praguecu},
F.~Tosello\Irefn{turin_i},
V.~Tskhay\Irefn{moscowlpi},
S.~Uhl\Irefn{munichtu},
B.I.~Vasilishin\Irefn{tomsk},
A.~Vauth\Irefn{cern},
B.M.~Veit\Irefn{mainz},
J.~Veloso\Irefn{aveiro},
A.~Vidon\Irefn{saclay},
M.~Virius\Irefn{praguectu},
M.~Wagner\Irefn{bonniskp},
S.~Wallner\Irefn{munichtu},
M.~Wilfert\Irefn{mainz},
K.~Zaremba\Irefn{warsawtu},
P.~Zavada\Irefn{dubna}, %20
M.~Zavertyaev\Irefn{moscowlpi},
Y.~Zhao\Irefn{triest_i},
E.~Zemlyanichkina\Irefn{dubna}\Aref{o}, %21
%N.~Zhuravlev\Irefn{dubna}, %22
M.~Ziembicki\Irefn{warsawtu}
\end{flushleft}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% institutes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{Authlist}
\item \Idef{alessandria}{Universita' degli Studi del Piemonte Orientale ``A. Avogadro'', Di.S.I.T., 15121 Alessandria, Italy}
\item \Idef{aveiro}{University of Aveiro, Dept.\ of Physics, 3810-193 Aveiro, Portugal}
\item \Idef{bochum}{Universit\"at Bochum, Institut f\"ur Experimentalphysik, 44780 Bochum, Germany\Arefs{l}\Aref{s}}
\item \Idef{bonniskp}{Universit\"at Bonn, Helmholtz-Institut f\"ur  Strahlen- und Kernphysik, 53115 Bonn, Germany\Arefs{l}}
\item \Idef{bonnpi}{Universit\"at Bonn, Physikalisches Institut, 53115 Bonn, Germany\Arefs{l}}
\item \Idef{brno}{Institute of Scientific Instruments, AS CR, 61264 Brno, Czech Republic\Arefs{m}}
\item \Idef{calcutta}{Matrivani Institute of Experimental Research \& Education, Calcutta-700 030, India\Arefs{n}}
\item \Idef{dubna}{Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\Arefs{o}}
\item \Idef{freiburg}{Universit\"at Freiburg, Physikalisches Institut, 79104 Freiburg, Germany\Arefs{l}\Aref{s}}
\item \Idef{cern}{CERN, 1211 Geneva 23, Switzerland}
\item \Idef{liberec}{Technical University in Liberec, 46117 Liberec, Czech Republic\Arefs{m}}
\item \Idef{lisbon}{LIP, 1000-149 Lisbon, Portugal\Arefs{p}}
\item \Idef{mainz}{Universit\"at Mainz, Institut f\"ur Kernphysik, 55099 Mainz, Germany\Arefs{l}}
\item \Idef{miyazaki}{University of Miyazaki, Miyazaki 889-2192, Japan\Arefs{q}}
\item \Idef{moscowlpi}{Lebedev Physical Institute, 119991 Moscow, Russia}
\item \Idef{munichtu}{Technische Universit\"at M\"unchen, Physik Dept., 85748 Garching, Germany\Arefs{l}\Aref{r}}
\item \Idef{nagoya}{Nagoya University, 464 Nagoya, Japan\Arefs{q}}
\item \Idef{praguecu}{Charles University in Prague, Faculty of Mathematics and Physics, 18000 Prague, Czech Republic\Arefs{m}}
\item \Idef{praguectu}{Czech Technical University in Prague, 16636 Prague, Czech Republic\Arefs{m}}
\item \Idef{protvino}{State Scientific Center Institute for High Energy Physics of National Research Center `Kurchatov Institute', 142281 Protvino, Russia}
\item \Idef{saclay}{IRFU, CEA, Universit\'e Paris-Saclay, 91191 Gif-sur-Yvette, France\Arefs{s}}
\item \Idef{taipei}{Academia Sinica, Institute of Physics, Taipei 11529, Taiwan\Arefs{tw}}
\item \Idef{telaviv}{Tel Aviv University, School of Physics and Astronomy, 69978 Tel Aviv, Israel\Arefs{t}}
\item \Idef{triest_u}{University of Trieste, Dept.\ of Physics, 34127 Trieste, Italy}
\item \Idef{triest_i}{Trieste Section of INFN, 34127 Trieste, Italy}
\item \Idef{turin_u}{University of Turin, Dept.\ of Physics, 10125 Turin, Italy}
\item \Idef{turin_i}{Torino Section of INFN, 10125 Turin, Italy}
\item \Idef{tomsk}{Tomsk Polytechnic University,634050 Tomsk, Russia\Arefs{nauka}}
\item \Idef{illinois}{University of Illinois at Urbana-Champaign, Dept.\ of Physics, Urbana, IL 61801-3080, USA\Arefs{nsf}}
\item \Idef{warsaw}{National Centre for Nuclear Research, 00-681 Warsaw, Poland\Arefs{u}}
\item \Idef{warsawu}{University of Warsaw, Faculty of Physics, 02-093 Warsaw, Poland\Arefs{u}}
\item \Idef{warsawtu}{Warsaw University of Technology, Institute of Radioelectronics, 00-665 Warsaw, Poland\Arefs{u} }
\item \Idef{yamagata}{Yamagata University, Yamagata 992-8510, Japan\Arefs{q} }
\end{Authlist}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Notes
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\theenumi{\alph{enumi}}
\begin{Authlist}
\item [{\makebox[2mm][l]{\textsuperscript{\#}}}] Corresponding authors
\item [{\makebox[2mm][l]{\textsuperscript{*}}}] Deceased
\item \Adef{a}{Also at Instituto Superior T\'ecnico, Universidade de Lisboa, Lisbon, Portugal}
\item \Adef{b}{Also at Dept.\ of Physics, Pusan National University, Busan 609-735, Republic of Korea and at Physics Dept., Brookhaven National Laboratory, Upton, NY 11973, USA}
\item \Adef{ictp}{Also at Abdus Salam ICTP, 34151 Trieste, Italy}
\item \Adef{r}{Supported by the DFG cluster of excellence `Origin and Structure of the Universe' (www.universe-cluster.de) (Germany)}
\item \Adef{p2i}{Supported by the Laboratoire d'excellence P2IO (France)}
\item \Adef{fuchey_adr}{Present address:  University of Connecticut, Storrs, Connecticut 06269, US}
\item \Adef{joerg_adr}{Present address: Universit\"at Bonn, Physikalisches Institut, 53115 Bonn, Germany}
\item \Adef{d}{Also at Chubu University, Kasugai, Aichi 487-8501, Japan\Arefs{q}}
\item \Adef{x}{Also at Dept.\ of Physics, National Central University, 300 Jhongda Road, Jhongli 32001, Taiwan}
\item \Adef{e}{Also at KEK, 1-1 Oho, Tsukuba, Ibaraki 305-0801, Japan}
\item \Adef{g}{Also at Moscow Institute of Physics and Technology, Moscow Region, 141700, Russia}
%\item \Adef{v}{Supported by Presidential Grant NSh--999.2014.2 (Russia)}
\item \Adef{h}{Present address: RWTH Aachen University, III.\ Physikalisches Institut, 52056 Aachen, Germany}
\item \Adef{yerevan}{Also at Yerevan Physics Institute, Alikhanian Br. Street, Yerevan, Armenia, 0036}
\item \Adef{y}{Also at Dept.\ of Physics, National Kaohsiung Normal University, Kaohsiung County 824, Taiwan}
\item \Adef{regen}{Also at Institut f\"ur Theoretische Physik, Universit\"at T\"ubingen, 72076 T\"ubingen, Germany}
%\item \Adef{infn}{Also at \ref{LItriest_i})}
\item \Adef{turin_p}{Also at University of Eastern Piedmont, 15100 Alessandria, Italy}
\item \Adef{i}{Present address: Uppsala University, Box 516, 75120 Uppsala, Sweden}
\item \Adef{c}{    Supported by the DFG Research Training Group Programmes 1102 and 2044 (Germany)} %mail Horst Fischer 20/09/2016 11:08
%
% support institutes
%
\item \Adef{l}{    Supported by BMBF - Bundesministerium f\"ur Bildung und Forschung (Germany)}
\item \Adef{s}{    Supported by FP7, HadronPhysics3, Grant 283286 (European Union)}
\item \Adef{m}{    Supported by MEYS, Grant LG13031 (Czech Republic)}
\item \Adef{n}{    Supported by B.Sen fund (India)}
\item \Adef{o}{    Supported by CERN-RFBR Grant 12-02-91500}
\item \Adef{p}{\raggedright 
                   Supported by FCT - Funda\c{c}\~{a}o para a Ci\^{e}ncia e Tecnologia, COMPETE and QREN, Grants CERN/FP 116376/2010, 123600/2011 
                   and CERN/FIS-NUC/0017/2015 (Portugal)}
\item \Adef{q}{    Supported by MEXT and JSPS, Grants 18002006, 20540299, 18540281 and 26247032, the Daiko and Yamada Foundations (Japan)}
\item \Adef{tw}{   Supported by the Ministry of Science and Technology (Taiwan)}
\item \Adef{t}{    Supported by the Israel Academy of Sciences and Humanities (Israel)}
\item \Adef{nauka}{Supported by the Russian Federation  program ``Nauka'' (Contract No. 0.1764.GZB.2017) (Russia)}
\item \Adef{nsf}{  Supported by the National Science Foundation, Grant no. PHY-1506416 (USA)}
\item \Adef{u}{    Supported by NCN, Grant 2017/26/M/ST2/00498 (Poland)}
%
\end{Authlist}
%
%


